Unraveling the Airalo Ecosystem

In recent years, we have witnessed myriad flavours of Mobile Network Aggregators (MNAs) which exploit the coverage footprint of a handful of base operators to provide global mobile connectivity. Under the MNA model, emerging operators reap the benefits of network softwarization and virtualization, including eSIM technology or control/data-plane separation. This paper investigates an emergent MNA type - a thick MNA - that relies on multiple (core) base operators from different economies to provision eSIM profiles, while employing gateway functions to the public internet located outside the respective base operators' home country. Specifically, our work is the first to capture the intricacies of Airalo - a thick MNA that operates in 219 countries. Unlike other MNAs that our community scrutinized, we show that Airalo often decouples the geographical location of the public internet gateway from the native country of the base operator via IPX Hub Breakout (IHBO). To map Airalo's underlying infrastructure, we ran web-based measurements that 14 volunteers performed while traveling and using an Airalo eSIM on their personal devices. We further dive into Airalo's performance by running device-based measurements (speedtest, traceroute, video streaming, etc.) in 10 countries with rooted Android devices. Finally, we examine Airalo's pricing by monitoring its marketplace.

==> sections/prolific-census.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Prolific Census}
\label{sec:prolific}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}
%     \includegraphics[width = \linewidth]{\folder/prolific//sat_maps.pdf}
%     \caption{----.}
%     \label{fig:census}
% \end{figure}
Prolific~\cite{prolific} is an online crowdsourcing platform with more than 130,000 vetted testers. Prolific offers powerful prescreening APIs for recruiting testers based on demographics, location, and even Internet Service Provider (ISP). ISP-based prescreening is only available for testers located in the US and the UK, where Prolific claims to be capable of correctly verifying ISP information~\cite{prolific-blog}.

\mvnote{Q: is airalo even listed?}
Currently, Prolific does not offer prescreening for eSIM users or Airalo customers. Intuitively, it can be hard for Prolific to constantly verify how their testers are connected. For example, a tester can create an account at home but then participate in surveys from her phone or from work. However, we suspect that some Prolific users might use eSIMs and Airalo as a connectivity mean. 

Accordingly, we created multiple measurement campaigns which leverage Prolific prescreening just to request \textit{mobile} users, but then explain in the study description that we are recruiting only testers with an active Airalo provided data plan. Users who accept to participate in our survey are then redirected to our website at \textit{------}. 

After loading our website, survey participant are instructed on how to take a screenshot of their currently active eSIM with Airalo. We then analyze suych screenshot using GPT vision to 1) verify an active Airalo users, 2) collect XX and YY information. If the Airalo connectivity is verified, the user is allowed to proceed with the second step. This step consists in performing a speedtest and uploading its result back to us. We use \textit{fast.com} since it can be loaded in an iframe inside our page, differently from cloudflare and speedtest, which avoid having the user opening a new tab. Since JS injection inside the iframe is not allowed, we again ask the user to upload a screenshot when the test is completed and ``more information is clicked''. 

Finally, we ask the user to comment on their Airalo experience with respect to its convenience, performance, and privacy, aka if they trust the service or notice any suspicious behavior. 
